Defending Against Data Reconstruction Attacks in Federated Learning: An Information Theory Approach

Federated Learning (FL) trains a black-box and high-dimensional model among different clients by exchanging parameters instead of direct data sharing, which mitigates the privacy leak incurred by machine learning. However, FL still suffers from membership inference attacks (MIA) or data reconstruction attacks (DRA). In particular, an attacker can extract the information from local datasets by constructing DRA, which cannot be effectively throttled by existing techniques, e.g., Differential Privacy (DP). In this paper, we aim to ensure a strong privacy guarantee for FL under DRA. We prove that reconstruction errors under DRA are constrained by the information acquired by an attacker, which means that constraining the transmitted information can effectively throttle DRA. To quantify the information leakage incurred by FL, we establish a channel model, which depends on the upper bound of joint mutual information between the local dataset and multiple transmitted parameters. Moreover, the channel model indicates that the transmitted information can be constrained through data space operation, which can improve training efficiency and the model accuracy under constrained information. According to the channel model, we propose algorithms to constrain the information transmitted in a single round of local training. With a limited number of training rounds, the algorithms ensure that the total amount of transmitted information is limited. Furthermore, our channel model can be applied to various privacy-enhancing techniques (such as DP) to enhance privacy guarantees against DRA. Extensive experiments with real-world datasets validate the effectiveness of our methods.

==> article/analysis.tex <==
\section{Analysis of Existing Methods} \label{sec:analysis_exist_method}

In this section, with our qualitative model, we aim at analyzing classical methods in CL for privacy preservation, such as differential privacy, gradient compression, and utilizing large batch size. Based on the perspective of information theory, we discover such methods in CL essentially reduce the risk of information leakage by decreasing the channel capacity $C^{(t)}$.

\subsection{Differential Privacy}

\begin{figure*}[tb]
%\vskip 0.1in
\begin{center}
\begin{minipage}[b]{0.32\textwidth}
\vskip -0.1in
\includegraphics[width=\textwidth]{graph/Rel_Dim.pdf}
\vskip -0.1in
\caption{If $\|\vg\|_2$ is upper bounded, $u_{\sigma}(d)$ increases as the dimension $d$ growing large, which implies a high dimensional gradient can encode more information.}\label{fig:Rel_Dim}
\vskip -0.2in
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\textwidth}
\vskip -0.1in
\includegraphics[width=\textwidth]{graph/Rel_Compre_Noise.pdf}
\vskip -0.1in
\caption{An example of gradient compression or sparsification, if we utilize gradient compression, it's equal to add more noise to the original gradient.}\label{fig:Rel_Compre_Noise}
\vskip -0.2in
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\textwidth}
\vskip -0.1in
\includegraphics[width=\textwidth]{graph/Rel_Batch_Size.pdf}
\vskip -0.1in
\caption{The relationship between channel capacity $C^{(t)}$ and the batch size. Moreover, with noise addition, $C^{(t)}$ is a decreasing function of batch size $B$. }\label{fig:Rel_Batch_Size}
\vskip -0.2in
\end{minipage}
\end{center}
\end{figure*}

As an important mechanism for data privacy, differential privacy, which mainly focuses on the problem of anonymization, is getting lots of attention in recent years. Specifically, in machine learning scenario as \cite{DBLP:conf/ccs/AbadiCGMMT016}, a typical process for $(\epsilon, \delta)$-DP can be formalized as two stages: gradient clipping, which guarantees the upper bound of sensitivity, and noise addition, which provides a $(\epsilon, \delta)$-DP based on the upper bounded sensitivity. However, in our qualitative model, the meaning of such two stages are different. On the one hand, gradient clipping puts a restriction on $\lambda^{(t)}_{i}$ in Eq.~(\ref{eq:info_func}), which represents the signal information. On the other hand, noise addition increases the noise component by increasing $\sigma^{(t)}$. Hence, from the perspective of information theory, $(\epsilon, \delta)$-DP actually guarantees that the channel capacity $C^{(t)}$ is upper bounded.

Specifically, on the first stage, if we denote the threshold of gradient clipping as $S$, then we get $\| \vg^{(t)} \|_2 \leq S$, where $\vg^{(t)}=\nabla_{\rmW}F(\rmW^{(t)}_{i};\; \rmD)$ is a random vector as a function of $\rmD$. Hence, we have
$$ \tr(\mSigma^{(t)}) \leq \tr(\mathE(\vg^{(t)}(\vg^{(t)})^{T}))=\mathE(\| \vg^{(t)} \|^2_2) \leq S^2, $$
where in the first inequality, we use the relationship between covariance matrix and the auto-correlation matrix: $\tr[\mathE(\vg^{(t)}(\vg^{(t)})^{T})-\mSigma^{(t)}] = \tr[\mathE(\vg^{(t)})\mathE(\vg^{(t)})^{T})]\geq 0$. Hence we have $\sum_{i=1}^{d}\lambda^{(t)}_i=\tr(\mSigma^{(t)})\leq S^2$. Then based on AM-GM inequality and the fact $\lambda^{(t)}_i\geq 0$, Eq.~(\ref{eq:info_func}) achieves its maximum when the eigenvalues, i.e., $\lambda^{(t)}_i, \; i=1, \cdots, d$, are identical with each other, which is
$$f^{(t)}(\sigma) \leq \hat{f}^{(t)}(\sigma)=d\cdot \ln\frac{\sigma+\frac{\sum_{i=1}^{d}\lambda^{(t)}_i}{d}}{\sigma} \leq d\cdot \ln\frac{\sigma+S^2/d}{\sigma}. $$
Therefore, if we treat $\sigma$ as a constant, and denote $u_{\sigma}(d) := d\cdot \ln\frac{\sigma+S^2/d}{\sigma}, d \geq 0$, we have $f^{(t)}(\sigma)\leq u_{\sigma}(d)$. Regarding $u_{\sigma}(d)$, we observe that $u^{'}_{\sigma}(d) = \ln\frac{\sigma+S^2/d}{\sigma} + \frac{\sigma}{\sigma+S^2/d}-1$, and its easy to verify
$$u{''}_{\sigma}(d)=-\frac{S^2(2\sigma d + S^2)}{d(\sigma d + S^2)^2} \leq 0 \Rightarrow u^{'}_{\sigma}(d)\geq u^{'}_{\sigma}(+\infty)=0,$$
which implies $u_{\sigma}(d)$ is an increasing function of the dimension $d$ (as illustrated in Fig.~\ref{fig:Rel_Dim}). Then based on L'Hospital's rule, we can conclude that
\begin{equation}\label{eq:channel_capacity_inf}
  C^{(t)}=f^{(t)}(\sigma)\leq u_{\sigma}(d) \leq u_{\sigma}(+\infty)=\frac{S^2}{\sigma}.
\end{equation}
Particularly, Eq.~(\ref{eq:channel_capacity_inf}) indicates the relationship between $C^{(t)}$ and the clipping bound $S$.

On the second stage, for a $(\epsilon, \delta)$-differentially private step, the authors in \cite{DBLP:journals/fttcs/DworkR14} demonstrate that we need to choose $\sigma \geq S^2\cdot \frac{2\log(1.25/\delta)}{\epsilon^2}$, then with a substitution in Eq.~(\ref{eq:channel_capacity_inf}), we have $C^{(t)}\leq \frac{\epsilon^2}{2\log(1.25/\delta)}$. Hence, $(\epsilon, \delta)$-DP in CL scenario guarantees that the channel capacity is upper bounded by $\frac{\epsilon^2}{2\log(1.25/\delta)}$.

\subsection{Gradient Compression}
As for gradient compression, based on the intuition, it's easy to understand such a compression mechanism decreases the information contained in the gradients, and we will formalize such an intuition with our qualitative model.

On the one hand, in the eigenspace of $\mSigma^{(t)}$, the channel capacity is $C^{(t)}=\frac{1}{2}\sum_{i=1}^{d}\ln\frac{\lambda^{(t)}_i + \sigma}{\sigma}$, and due to the non-negativity of $\lambda^{(t)}_i$, $\ln\frac{\lambda^{(t)}_i + \sigma}{\sigma}\geq 0$, $i\in\{1,\cdots,d\}$, represents the upper bound of information contained in the different independent dimensions. As illustrated in Fig.~\ref{fig:Rel_Compre_Noise}, if we set a positive $\lambda^{(t)}_i$ to be $0$, then the corresponding $C^{(t)}$ decreases, and the capacity drops even more as the corresponding $\lambda^{(t)}_i$ increases. Moreover, compared to the noise strategy, with regard to the channel capacity, the more information compression is equivalent to the lager noise addition.

On the other hand, in practice, the gradient compression always works on the gradient $\vg$ directly \cite{DBLP:conf/iclr/LinHM0D18,DBLP:conf/iclr/TsuzukuIA18}, hence we need to analyze $\mSigma^{(t)}$ itself. Specifically, the information contained in different dimensions are not independent any more, then without loss of generality, we can rewrite $\mSigma^{(t)}$ as
  \begin{align}\label{matrix_decomp}
  \mSigma^{(t)} = &\left( \begin{array}{cc}
                              \mP_{d-k} & \mR \\
                              \mR^{\mathrm{T}}    & \mQ_{k}
                            \end{array}\right) \\ = &\left( \begin{array}{cc}
                                                           \mI_{d-k} & \mathbf{0} \notag \\
                                                           \mR^{\mathrm{T}}  \mP_{d-k}^{-1} & \mI_{k}
                                                         \end{array} \right)\left( \begin{array}{cc}
                                                                                     \mP_{d-k} & \mR \\
                                                                                     \mathbf{0} & \mQ_{k}-\mR^{\mathrm{T}}\mP_{d-k}^{-1}\mR
                                                                                   \end{array}\right),
  \end{align}
where $\mP_{d-k}\in \mathbb{R}^{(d-k)\times (d-k)}$ represents the covariance matrix of the uncompressed dimension, $\mQ_{k}\in \mathbb{R}^{k\times k}$ represents the covariance matrix of the compressed dimension, and $\mR \in \mathbb{R}^{(d-k)\times k}$ represents the mutual covariance matrix between the compressed dimension and the uncompressed dimension. Thus, we have
\begin{equation}\label{eq:model_compression}
  \det(\mSigma^{(t)}) = \det(\mP_{d-k})\cdot\det(\mQ_{k}-\mR^{\mathrm{T}}\mP_{d-k}^{-1}\mR).
\end{equation}
Hence, combined Eq.~(\ref{eq:model_compression}) with Thm.~\ref{thm:channel_capacity}, we can conclude the channel capacity decrease caused by compression can be formalized as
$$\Delta C^{(t)}=\frac{1}{2}\ln\frac{\det(\mQ_{k}+\sigma\mI_{k}-\mR^{\mathrm{T}}(\mP_{d-k}+\sigma\mI_{d-k})^{-1}\mR)}{\sigma^k}$$

\subsection{Large Batch Size}

Another defense strategy for deep leakage in CL scenarios is large batch size \cite{DBLP:conf/nips/ZhuLH19}, which makes the leakage more difficult via entangling the information contained in multiple data points. However, with our qualitative model, such a strategy is easy to be formalized. Specifically, we denote the batch size as $B$, then the gradients in mini-batch SGD is $ \frac{1}{B}\sum_{i=1}^{B}\nabla_{\rmW}F(\rmW^{(t)}_{i};\; \rmD_i)$, where $\rmD_i$ represents the iid random variables, and the covariance matrix with large batch size is scaled by $B$, i.e., $\mSigma^{(t)}_B=\frac{1}{B}\mSigma^{(t)}$. Hence based on Thm.~\ref{thm:channel_capacity} and the substitution with $\mSigma^{(t)}_B$ for $\mSigma^{(t)}$, we have
$$ C^{(t)}_B = f_B^{(t)}(\sigma) := \frac{1}{2}\ln\frac{\prod_{i=1}^{d}(\lambda^{(t)}_i + B\sigma)}{(B\sigma)^{d}}, $$
hence, the batch size is a multiplicative coefficient. Moreover, as illustrated in Fig~\ref{fig:Rel_Batch_Size}, with noise addition, $C^{(t)}$ is a decreasing function of $B$.
%In the previous section, we discussed the mutual information between the dataset and the in\&out information flow, which is mainly related to the information leakage in collaborative leaning. Then the problem is narrowed down to the information control in a typical communication round, which depends on the aforementioned internal flow, and we will solve the problem of information control in this section.
%
%Before proposing the method of information control, we need to make an extension of Thm \ref{one_step_mi} and the corresponding corollary from discrete to continuous. When dealing with the case of continuous, we need to change the discrete entropy $H(\rmX)$ to differential entropy $h(\rmX)$, and the situation is slightly different: $h(\rmW_{o,t} \;|\; \rmD, \; \rmW_{i,t}=\rvw_{i,t})$ is not $0$ due to the property of differential entropy. Indeed, $h(\rmW_{o,t} \;|\; \rmD, \; \rmW_{i,t}=\rvw_{i,t}) \to -\infty$ as $\rmW_{o,t}$ is deterministic when $\rmW_{i,t}$ and $\rmD$ are both observed. This is reasonable since the volume of the support set goes into $0$ when the variable is deterministic, and $2^{-\infty}=0$ either (as illustrated in \cite{DBLP:books/daglib/0016881}). Then the mutual information between the egress flow and the local dataset $I(\rmD, \; \rmW_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \to +\infty$, and we will discuss it later in this section. However, as the continuous mutual information is the limit of discrete one, most of properties are preserved, hence the rest theorems and corollaries in the previous section remain the same in the continuous situation.
%
%As afore mentioned, due to the property of differential entropy, the mutual information is $+\infty$ when $\rmW_{o,t}$ is deterministic, and it brings difficulties for information analysis. To resolve this dilemma, we need to introduce an random variable and turn to analysis $\widetilde{\rmW}_{o,t} = \rmW_{o,t}+\sqrt{\sigma} \cdot \bf{\xi}$, where $\sigma \geq 0$ and $\bf{\xi}\sim \mathN(\bf{0},\; \rmI)$. Note that $\widetilde{\rmW}_{o,t}$ represents a noisy egress flow, a typical method for privacy protection in collaborative learning. And in such circumstance, $\rmW_{o,t}=\lim\limits_{\sigma \to 0}\widetilde{\rmW}_{o,t}$. An important property of $\widetilde{\rmW}_{o,t}$ is implied as following lemma.
%
%\begin{lemma}\label{lemma:upper_bound_entropy}
%  For a continuous random variable $\rmX$ with $\mathE[\rmX] = \vmu_{\rmX}$, $Cov(\rmX) = \mSigma_{\rmX}$ and an independent Gaussian random variable $\rmY \sim \mathN(\vmu_{\rmY}, \;\mSigma_{\rmY})$, $h(\rmX+\rmY)$ achieves its maximum when $\rmX \sim \mathN(\vmu_{\rmX}, \;\mSigma_{\rmX})$.
%\end{lemma}
%\begin{proof}
%  Firstly, as $\rmX$ and $\rmY$ are independent, then $\mathE[\rmX+\rmY] = \vmu_{\rmX} + \vmu_{\rmY}$ and $Cov(\rmX+\rmY) = \mSigma_{\rmX} + \mSigma_{\rmY}$. Secondly, with a specific mean vector and covariance matrix, the maximum entropy distribution is Gaussian, which implies that $h(\rmX+\rmY) \leq h(\mathN(\vmu_{\rmX} + \vmu_{\rmY}, \; \mSigma_{\rmX} + \mSigma_{\rmY}))$. Finally, if $\rmX \sim \mathN(\vmu_{\rmX}, \;\mSigma_{\rmX})$, then $\rmX+\rmY \sim \mathN(\vmu_{\rmX} + \vmu_{\rmY}, \; \mSigma_{\rmX} + \mSigma_{\rmY})$, which concludes the proof.
%\end{proof}
%
%Lemma \ref{lemma:upper_bound_entropy} implies we can restrict corresponding differential entropy by limiting its upper bound with Gaussian distribution. Then we can derive our main theorem for information controlling.
%
%\begin{theorem}\label{thm:channel_capacity}
%  Let $\widetilde{\rmW}_{o,t} = \rmW_{o,t}+\sqrt{\sigma} \cdot \bf{\xi}$, where $\sigma \geq 0$ and $\bf{\xi}\sim \mathN(\bf{0},\; \rmI)$, if $\vmu$ and $\mSigma$ are the mean vector and covariance matrix of $\rmW_{o,t}$ respectively when $\rmW_{i,t}$ is observed, then we have $I(\rmD, \; \widetilde{\rmW}_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \leq f(\sigma)$, where $f(\sigma)$ is defined as follows:
%  \begin{equation}\label{eq:info_func}
%    f(\sigma) := \frac{1}{2}\ln\frac{\prod_{i=1}^{d}(\lambda_i + \sigma)}{\sigma^{d}}, \; \sigma \in (0, \; +\infty).
%  \end{equation}
%  $\lambda_i$ is the i-th eigenvalue of covariance matrix $\mSigma$ and $d$ represents the dimension of $\rmW_{o,t}$.
%\end{theorem}
%
%\begin{proof}
%  According to the relationship between mutual information and differential entropy,
%  \begin{align}
%    &I(\rmD, \; \widetilde{\rmW}_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \notag\\
%    =&  h(\widetilde{\rmW}_{o,t} \;| \; \rmW_{i,t}=\rvw_{i,t}) - h(\widetilde{\rmW}_{o,t} \;|\; \rmD, \; \rmW_{i,t}=\rvw_{i,t}) \notag\\
%                                                                    = & h(\widetilde{\rmW}_{o,t} \;| \; \rmW_{i,t}=\rvw_{i,t}) - h(\mathN(\bf{0},\; \sigma \cdot \rmI)) \notag\\
%                                                                    \leq & h(\mathN(\vmu,\; \mSigma + \sigma \cdot \rmI))-h(\mathN(\bf{0},\; \sigma \cdot \rmI)), \label{upper_bound_gaussian}
%  \end{align}
%  where the second equality depends on determinacy of $\rmW_{o,t}$ when $\rmW_{i,t}$ and $\rmD$ are both observed, and the last inequality is an immediate consequence of Lemma \ref{lemma:upper_bound_entropy} with $\widetilde{\rmW}_{o,t} = \rmW_{o,t}+\sqrt{\sigma} \cdot \bf{\xi}$.
%
%  Then with the differential entropy of Gaussian distribution, we can further transform formula (\ref{upper_bound_gaussian}) to
%  \begin{align}\label{Gaussian_det}
%      &h(\mathN(\vmu,\; \mSigma + \sigma \cdot \rmI))-h(\mathN(\bf{0},\; \sigma \cdot \rmI)) \notag\\
%       = &\frac{1}{2} \ln \det(\mSigma + \sigma \cdot \rmI) - \frac{1}{2}\ln \sigma^d,
%  \end{align}
%  where $\det(\cdot)$ denotes the determinant of a matrix and the second term on the right side is determined by $\det(\sigma \cdot \rmI) = \sigma^d$.
%
%  Next, we focus on the first term of Eq. \ref{Gaussian_det}. Note that $\mSigma$ is the covariance matrix of $\rmW_{o,t}$, hence it's a real symmetric matrix, then according to spectral decomposition,
%  $$ \mSigma = \rmQ \bf{\Lambda} \rmQ^T = \rmQ \cdot \mathrm{diag}(\lambda_1, \cdots, \lambda_d ) \cdot \rmQ^\mathrm{T},$$
%  where $\rmQ$ is an orthogonal matrix, i.e., $\rmQ \rmQ^\mathrm{T} = \rmI$. Based on the property of orthogonal matrix, $\sigma \cdot \rmI = \rmQ \cdot(\sigma \rmI) \cdot \rmQ^\mathrm{T} $. Hence,
%  \begin{align*}
%    \det(\mSigma + \sigma \cdot \rmI) & = \det(\rmQ \cdot \mathrm{diag}(\lambda_1, \cdots, \lambda_d ) \cdot \rmQ^\mathrm{T} + \rmQ \cdot(\sigma \rmI) \cdot \rmQ^\mathrm{T}) \\
%                                      & = \det(\mathrm{diag}(\lambda_1, \cdots, \lambda_d )+\sigma \rmI) = \prod_{i=1}^{d}(\lambda_i + \sigma).
%  \end{align*}
%  Then we have $I(\rmD, \; \widetilde{\rmW}_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \leq \frac{1}{2}\ln\frac{\prod_{i=1}^{d}(\lambda_i + \sigma)}{\sigma^{d}}$, which immediately completes the proof.
%\end{proof}

%As afore mentioned, $I(\rmD, \; \widetilde{\rmW}_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} )$ denotes a noisy communication channel, which introduce noisy strategy to protect the local privacy. Then based on Thm \ref{thm:info_ctr}, we can further investigate the performance of such strategy by analysing the property of its upper bound $f(\sigma)$. Indeed, according to Centre Limit Thorem, if we choose mini-batch stochastic gradient descent, the distribution of $\rmW_{o,t}$ approximate to the Gaussian distribution as the batch growing large, which means the inequality becomes tighter with the increasing batch size.
%
%For information control, we need to analyse the property of $f(\sigma)$. First, we investigate the asymptotic property of $f(\sigma)$, in one direction, $\lim\limits_{\sigma \to 0}f(\sigma) = +\infty$, which is consistent with $I(\rmD, \; \rmW_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \to +\infty$; while in another direction, $\lim\limits_{\sigma \to +\infty}f(\sigma) = 0$, combine it with the non-negativity of mutual information, we can conclude that the strategy purely depends on noise need to introduce infinite noise to restrict the information leakage to be $0$. Then we try to analyse the monotonicity according to its derivative,
%$$ f'(\sigma) = \frac{1}{2}\sum_{i=1}^{d}\frac{-\lambda_i}{\sigma^2+\lambda_i \sigma}, $$
%since covariance matrix is a positive definite matrix, then its eigenvalue $\lambda_i > 0$, hence $f'(\sigma)<0$ as $\sigma$ is non-negative, which implies $f(\sigma)$ is a monotone decreasing function in its domain, i.e., the mutual information is decreasing as we add more noise into the output parameters $\rmW_{o,t}$, it's a property consistent with our intuition (as illustrated in Fig. \ref{fig:Rel_Dim}). Therefore, let $f(\sigma)=\epsilon$, there is an unique $\sigma$ satisfies $I(\rmD, \; \widetilde{\rmW}_{o,t} \;|\; \rmW_{i,t}=\rvw_{i,t} ) \leq \epsilon$. Finally, another interesting property of $f(\sigma)$ is that
%$$f''(\sigma) = \frac{1}{2}\sum_{i=1}^{d}\frac{2\lambda_i \sigma+\lambda^2_i}{(\sigma^2+\lambda_i \sigma)^2} > 0,$$
%$f''(\sigma)>0$ means $f(\sigma)$ is a convex function, and $|f'(\sigma)|$ decreases as $\sigma$ increases, which implies the property of diminishing marginal utility for noise strategy. 

==> article/intro.tex <==
\section{Introduction}
Federated learning (FL)~\cite{DBLP:conf/aistats/McMahanMRHA17,DBLP:journals/tist/YangLCT19}  is a new form of machine learning (ML),
which protects privacy by transmitting gradients or parameters to avoid sharing raw data. Specifically, the parameters form a \emph{communication channel} between the server and each client, so the server gets information from local datasets via such channels. Based on the Data Processing Inequality (DPI) \cite{DBLP:books/daglib/0016881}, communication by parameters, which is a deterministic mapping of local data, instead of raw data, reduces the risk of data privacy.
%(illustrated in the second layer in Fig.~\ref{fig:overview_infoflow}).
%Furthermore, when we step into the data driven age, such a strategy with data protection removes part of barriers to gather information from different clients so as to improve AI service, leading to more social profit.

% \begin{figure}[tb]
% %\vskip 0.1in
% \begin{center}
% \begin{minipage}[b]{\columnwidth}
% %\vskip -0.1in
% \includegraphics[width=\columnwidth]{graph/OverView.pdf}
% \vskip -0.1in
% \caption{In this work, we demonstrate that the reconstruction error of DRA can be constrained above a certain threshold. Given a dataset $\mD$, our techniques provide a lower bound $d_{*}$ for the reconstruction error by deciding the covariance matrix $\mSigma_{*}$ for the adding noise.}\label{fig:overview_infoflow}
% \end{minipage}
% \vskip -0.5in
% \end{center}
% \end{figure}

% \footnotetext[1]{Mutual information, which represents the reduction of randomness for data $\mD$ if we observe $\mW$, i.e., the knowledge increment about $\mD$.}
%\cite{DBLP:journals/corr/abs-2211-03128}.
%However, the communication channel formed by parameters is still not secure enough
However, recent studies reveal that the parameter channel of FL still leaks privacy.
For example,
%Recent literatures \cite{DBLP:conf/icml/SablayrollesDSO19,DBLP:conf/sp/NasrSH19, DBLP:conf/eurosp/LongWBB0TGC20,DBLP:conf/icml/Choquette-ChooT21,DBLP:conf/sp/CarliniCN0TT22} indicate that
multiple literature indicates that adversaries can conduct membership inference attacks (MIA) with uploaded model parameters~\cite{DBLP:conf/icml/SablayrollesDSO19,DBLP:conf/sp/NasrSH19,DBLP:conf/sp/MelisSCS19,DBLP:conf/eurosp/LongWBB0TGC20,DBLP:conf/icml/Choquette-ChooT21,DBLP:conf/sp/CarliniCN0TT22}, which breaks the anonymity of data privacy. Moreover, adversaries can completely steal training data by data reconstruction attacks (DRA)~\cite{DBLP:conf/ccs/HitajAP17,DBLP:conf/nips/ZhuLH19,DBLP:conf/uss/CarliniTWJHLRBS21,DBLP:conf/nips/HaimVYSI22}, resulting in serious privacy issues in FL.

Existing studies mainly utilize dimension reduction~\cite{DBLP:conf/kdd/LiDYC020, DBLP:journals/tkde/OsiaTSKHR20,DBLP:conf/aaai/ThapaCCS22} or Differential Privacy (DP) \cite{DBLP:conf/nips/AgarwalSYKM18,DBLP:conf/sosp/LecuyerSVG019,DBLP:conf/nips/LevySAKKMS21} to enhance the \qi{privacy protection in FL. However, \yi{dimension reduction} lacks theoretical guarantees of the defense ability against DRA, while \yi{DP} still suffers from the \yi{issue} of data reconstruction even with theoretical guarantees \cite{DBLP:conf/kdd/Cormode11, DBLP:conf/uss/LiuWH000CF022,DBLP:journals/corr/abs-2302-07225,DBLP:conf/sp/BalleCH22,DBLP:conf/icml/GuoKCM22}. Additionally, literature \cite{DBLP:conf/sp/BalleCH22,DBLP:conf/icml/GuoKCM22} indicates DP's theory primarily focuses on MIA, hence conventional DP variables (e.g., the privacy budget $\epsilon$) are insufficient in describing the capability of defending against DRA. For instance, in DP-SGD \cite{DBLP:conf/sp/BalleCH22}, algorithms with identical DP guarantees but different hyper-parameters cannot guarantee the same success rate for DRA. Both of them
%can still be
\yi{remain}
vulnerable to DRA.}

%In a nutshell, the theories for defending against DRA have not been thoroughly investigated.
To establish a theoretical foundation for DRA, we demonstrate that the lower bound of mean squared error (MSE), which serves as an indicator of DRA's precision in reconstruction (i.e., the smaller MSE means the higher precision for the attacker), is determined by the amount of acquired information, i.e., the mutual information (MI)\footnote{Mutual information $I(X;Y)$ \cite{DBLP:conf/ccs/CuffY16,DBLP:journals/corr/Shwartz-ZivT17,DBLP:conf/iclr/HjelmFLGBTB19} represents the uncertainty decrement of $X$ when we observe $Y$.} between the local dataset and the shared parameters. Specifically, the smaller MI results in a larger MSE, indicating that it is more difficult for an attacker to reconstruct the local dataset. \qi{In other words, MI can be utilized as the indicator for quantifying the information leakage in FL. As a result, the goal for defending against DRA is to restrict the MI between the local dataset and the transmitted parameters.}

%which inspires us to formalize the issue of privacy leakage in FL by information theory.

% \qi{An important aspect of quantifying the information leakage is the kind of attack that we want to model \cite{DBLP:conf/ccs/0002CPP20}.
%Traditional theory like
\qi{However, previous techniques for quantifying information leakage cannot be applied to analyze DRA in the FL scenario. For example, Quantitative Information Flow (QIF) \cite{DBLP:series/isc/AlvimCMMPS20} quantifies information leak under a white-box and time-invariant setting\cite{DBLP:conf/ccs/0002CPP20}. It requires the knowledge of the correlation between the distributions of inputs and outputs, which cannot hold in FL systems. In fact, FL always trains a black-box and high dimensional model (e.g., deep neural networks), and the iterative training process makes the model to be time-variant. Hence, QIF cannot directly be applied to the FL scenario. Moreover, QIF focuses on a special security concern, namely the probability of guessing a secret in one try~\cite{DBLP:series/isc/AlvimCMMPS20,DBLP:conf/fossacs/Smith09}. This security concern is different from the one in DRA, where DRA focuses on reconstructing the whole distribution of local data. %Specifically, the black-box issue causes difficulties to model the output distribution in FL, while the high dimensional and time-variant model incurs huge amount of calculation for the model processing. 
Therefore, we build a quantitative model to analyze information leaks under the black-box setting.
%which quantifies the transmitted information in FL as the accumulation of MI between the local dataset and shared parameters. %Guided by the model,
\yi{Through our proposed quantitative model,}
we
%discover
\yi{find}
that the transmitted information (i.e., the information leakage) is decided by two factors: the channel capacity $C$, which represents the maximal ability for transmitting information in a single training round; and the optimization rounds $n$, which is correlated to the information accumulation.
For example, if the channel capacity is upper bounded by a threshold $\kappa$, and the number of optimization rounds is less than $n$, then the total amount of information leakage is less than $n \cdot \kappa$. Furthermore, our proposed quantitative model can be used to analyze various methods, including DP, gradient compression, and utilizing large batch size.}
%Hence, reducing channel capacity and limiting communication rounds are the fundamental strategies to strengthen the capabilities for defending against DRA.

%Particularly, the model provides theoretical guarantees in protecting against DRA for various methods, including DP, gradient compression, utilizing large batch size, etc.

\qi{Based on the quantitative model, we utilize DPI to transform the operations (e.g., eigen-decomposition and adding noise) of constraining channel capacity from the parameter space to the data space. This transformation significantly improves both the training efficiency and the model accuracy of the high dimensional and time-variant model in FL.}
Specifically, our \emph{protecting goal} is to decide the covariance matrix for the added noise according to a given data distribution $\mD$, which ensures privacy protection by constraining the reconstruction error above a certain threshold. Compared to conventional protection techniques, which directly deal with parameters after gradient mapping, constraining in the data space has two distinct advantages:
firstly, it makes the computational complexity independent of the optimization rounds $n$ and the model's dimensionality $d_m$, reducing it from $\mathcal{O}(n\cdot d_m)$ to $\mathcal{O}(d_D)$, where $d_D$ denotes the dimensionality of the data and $d_D \ll d_m$. Secondly, data space preserves the correlations between data attributes, hence we can leverage the prior knowledge of relative importance to implement stronger safeguards for the critical attributes, which enhances the capability to balance the utility and the privacy. 

Finally, according to the theoretical results, we propose three implementation methods for constraining the channel capacity. These implementation methods incorporate different prior knowledge in defending against DRA, which can be employed to flexibly balance the utility and the privacy.
%Among them, Natural Channel keeps the original relative importance between different attributes, thus achieving better model accuracy. White Channel treats each attribute equally, which enhances the protection capability without prior knowledge. As for the Personalized Channel, it allows the client to leverage prior knowledge of attribute importance, thereby enabling flexible trade-offs between utility and privacy.

In summary, the contributions of our paper are as follows:
\begin{itemize}
\setlength{\itemsep}{2pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
  \item We demonstrate that the reconstruction error of DRA is lower bounded by the amount of acquired information.
  \item \qi{We establish a quantitative model to quantify the information leakage of the black-box model in FL, which can be applied to analyze various privacy-enhancing methods for defending against DRA.}
  \item \qi{We theoretically constraining the transmitted information through the operation in data space instead of parameter space for the first time and demonstrate that it significantly improves both the training efficiency and the model accuracy.}
  \item By incorporating different prior knowledge, we propose three implementations to constrain channel capacity, which can be utilized to flexibly balance the utility and the pravacy.
  \item \qi{Extensive experiments demonstrate that the newly proposed methods effectively enhance the safety, efficiency, and flexibility of FL.}
\end{itemize}

